SAVIOR: Towards Bug-Driven Hybrid Testing

Hybrid testing combines fuzz testing and concolic execution. It leverages fuzz testing to test easy-to-reach code regions and uses concolic execution to explore code blocks guarded by complex branch conditions. However, its code coverage-centric design is inefficient in vulnerability detection. First, it blindly selects seeds for concolic execution and aims to explore new code continuously. However, as statistics show, a large portion of the explored code is often bug-free. Therefore, giving equal attention to every part of the code during hybrid testing is a non-optimal strategy. It slows down the detection of real vulnerabilities by over 43%. Second, classic hybrid testing quickly moves on after reaching a chunk of code, rather than examining the hidden defects inside. It may frequently miss subtle vulnerabilities despite that it has already explored the vulnerable code paths. We propose SAVIOR, a new hybrid testing framework pioneering a bug-driven principle. Unlike the existing hybrid testing tools, SAVIOR prioritizes the concolic execution of the seeds that are likely to uncover more vulnerabilities. Moreover, SAVIOR verifies all vulnerable program locations along the executing program path. By modeling faulty situations using SMT constraints, SAVIOR reasons the feasibility of vulnerabilities and generates concrete test cases as proofs. Our evaluation shows that the bug-driven approach outperforms mainstream automated testing techniques, including state-of-the-art hybrid testing systems driven by code coverage. On average, SAVIOR detects vulnerabilities 43.4% faster than DRILLER and 44.3% faster than QSYM, leading to the discovery of 88 and 76 more uniquebugs,respectively.Accordingtotheevaluationon11 well fuzzed benchmark programs, within the first 24 hours, SAVIOR triggers 481 UBSAN violations, among which 243 are real bugs.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ ~* *.log *.gz *.aux *.dvi *.out *.bbl *.blg *.cb *.dep main.pdf
	rm -rf _minted-* 

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex -shell-escape #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> codelisting_src/Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ ~* *.log *.gz *.aux *.dvi *.out *.bbl *.blg *.cb *.dep $(TARGET)
	rm -rf _minted-*

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex -shell-escape #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> eval2.tex <==
\subsection{Application in Vulnerability Finding}
Besides evaluating the utility of the key techniques, 
we further applied \savior to hunt security defects in the wild. 
To date, we have covered the programs listed in Table~\ref{tab:eval-setup} 
and two well tested programs, {\tt lcms} and {\tt proj4}
Due to limit of computation resources and time, 
we only ran each program for 24 hours. In total, 
\savior triggered \TOTOALBUGNUM unique exceptions, 
among which \UBNUM are UBsan violations and \NONUBNUM
are non-UBSan bugs. The details are summarized in Table~\ref{tab:ub-bug}
and Table~\ref{tab:nonub-bug}. 
We have manually confirmed all non-UBSan bugs and we are 
examining all the UBSan violations. 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tcpdump-trigger.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf tcpdump}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tcpdump-bugcov1.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf tcpdump} (total UBSan labels: 13940).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tcpdump-codecov.pdf}
        \captionsetup{margin=0.5cm}
        \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf tcpdump} (total basic blocks: 65725).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2ps1.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf tiff2ps}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2ps-bugcov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf tiff2ps} (total UBSan labels: 2186).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2ps-codecov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf tiff2ps} (total basic blocks: 15691).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/readelf.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf readelf}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/readelf-bugcov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf readelf} (total UBSan labels: 2732).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/readelf-codecov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf readelf} (total basic blocks: 19311).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/libxml.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf libxml}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/libxml-bugcov.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf libxml} (total UBSan labels: 5324).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/libxml-codecov.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf libxml} (total basic blocks: 84153).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2pdf.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf tiff2pdf}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2pdf-bugcov.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf tiff2pdf} (total UBSan labels: 5324).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/tiff2pdf-codecov.pdf}
        \captionsetup{margin=0.5cm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf tiff2pdf} (total basic blocks: 84153).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
    %\caption{Evaluation results with real-world programs. \todo{briefly explain each column}}
    \label{fig:bugcovcont}
\end{figure*}
\begin{figure*}[t!]\ContinuedFloat
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jpeg.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf djpeg}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jpeg-bugcov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf djpeg} (total UBSan labels: 9414).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jpeg-codecov.pdf}
        \captionsetup{margin=0.5cm}
        \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf djpeg} (total basic blocks: 26442).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jasper.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf jasper}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jasper-bugcov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf jasper} (total UBSan labels: 2186).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/jasper-codecov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf jasper} (total basic blocks: 15691).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}\\
\iffalse
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/objdump.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations triggered in \emph{\bf objdump}.}}
        \label{fig:eval:fast:jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/objdump-bugcov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of UBSan violations reached in \emph{\bf objdump} (total UBSan labels: 9105).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=0.90\textwidth]{figs/eval/savior/objdump-codecov.pdf}
        \captionsetup{margin=0.5cm}
         \vspace*{-2mm}
        \caption{\scriptsize{Number of basic blocks reached in \emph{\bf objdump} (total basic blocks: 69957).}}
        \label{fig:eval:fast:catdoc}
    \end{subfigure}
\fi
    \caption{Evaluation results with real-world programs. The three columns respectively show the number of
    triggered UBSan labels, the number of reached UBSan labels, and the number of covered basic blocks by different 
    fuzzers over 24 hours.}
    \vspace{-2ex}
    \label{fig:eval-res-real}
\end{figure*}
example of false positive.
\begin{lstlisting}
char array[MAX]; // 0 < MAX < INT_MAX
for(int i = 0; i < MAX;){
    array[i] = getchar();//LABEL: OOB access 
    i++;//LABEL: integer-overflow
}
\end{lstlisting}
